Mutual Information-Empowered Task-Oriented Communication: Principles, Applications and Challenges

Mutual information (MI)-based guidelines have recently proven to be effective for designing task-oriented communication systems, where the ultimate goal is to extract and transmit task-relevant information for downstream task. This paper provides a comprehensive overview of MI-empowered task-oriented communication, highlighting how MI-based methods can serve as a unifying design framework in various task-oriented communication scenarios. We begin with the roadmap of MI for designing task-oriented communication systems, and then introduce the roles and applications of MI to guide feature encoding, transmission optimization, and efficient training with two case studies. We further elaborate the limitations and challenges of MI-based methods. Finally, we identify several open issues in MI-based task-oriented communication to inspire future research.

==> section/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

In this article, we have presented a series of practical challenges and initail solutions in designing efficient and robust task-oriented communication systems. We first introduced three training strategies 

Two case studies have shown the effectiveness of the proposed methods in improving the efficiency and robustness of task-oriented communication systems. We further discussed several open issues and research directions for future work.

==> section/future.tex <==
\section{Future directions and open issues}
Previous sections have discussed the practical challenges and corresponding initial solutions in designing efficient and robust task-oriented communication systems, several open issues and future directions are highlighted as follows.

\subsection{Advanced Techniques for Remote Training}
The remote training method is practical when the transmitter and receiver are physically separated, especially when only fine-tuning is required after deployment or combined with self-supervsied local training, like that introduced in Section~\ref{sec:method}. However, the frequent exchange of float numbers between the transmitter and receiver may incur high communication overhead. To address this issue, the design of efficient remote training methods is essential. Specifically, several efficient strategies like quantization, sparsification, and gradient compression to reduce the communication overhead of huge floating-point number can be explored.

\subsection{Convergence Analysis and System Optimization}
Ensuring fask and stable convergence is critical for the effectiveness of remote training in task-oriented communication systems, especially when the intermediate features and gradient information are transmitted over wireless channel. To this end, the quantitative convergence analysis of remote training in task-oriented communication systems is necessary, further optimization of the system design, such as the beamforming design, power allocation and precoding design, can be explored to improve the convergence performance.

\subsection{Co-Design of Communication and Learning}
We focus on efficient training and robust inference algorithm from DL perspective, in which the strategy can be applied to various communication systems. However, the co-design of communication and learning for more efficient and robust system can be further explored to improve the performance of task-oriented communication systems. For instance, the Maximal Coding Rate Reduction (MCR$^2$) method can be integrated with the proposed feature alignment strategy to improve the precoding design in MIMO systems. Specifically, the MCR$^2$ method can guide the learning process to optimize semantic feature extraction and alignment while simultaneously influencing the MIMO precoding design. This will not only align transceiver features for cross-transceiver communication but also leverage the spatial diversity of MIMO systems to improve transmission efficiency and reliability.


\subsection{Privacy and Security in Task-Oriented Communication Systems}
Privacy and security are critical challenges in task-oriented communication systems, as the exchange of intermediate features, gradient information or the model parameters can expose sensitive information to potential adversaries. To address these concerns, techniques such as differential privacy and homomorphic encryption can be employed to protect sensitive data during transmission and computation. Additionally, federated learning approaches can reduce privacy risks by exchanging model updates instead of raw data. On the security side, adversarial robustness mechanisms, including adversarial training and gradient masking, can safeguard the system from malicious attacks. Future research should focus on balancing privacy, security, and system efficiency, ensuring compliance with emerging privacy regulations and robust performance in dynamic and multi-user scenarios.

==> section/introduction.tex <==
\section{introduction}
\label{sec:introduction}
As Shannon and Weaver pointed out in their seminal work~\cite{shannon1948mathematical}, communication problems are identified as three levels: 1) technical problem, 2) semantic problem, and 3) effectiveness problem. Traditional communication systems have been focusing on solving the technical problem by transmitting the raw data with high fidelity. However, the huge demand for data delivering in the era of big data and artificial intelligence (AI) has an urgent need for solving the semantic problem and effectiveness problem, which can significantly improve the efficiency of communication systems. To this end, task-oriented communication has emerged as a pivotal enabler for next-generation wireless communication networks by focusing on the extraction and transmission of only necessary information for downstream tasks, which contrasts sharply with traditional communication systems that aims at delivering the raw data with high fidelity. To enable an efficient task-oriented communication system, the establation of shared knowledge base (KB) between transceivers is critical for transmitting only task-relevant information, as the KB contains the consensus information that can guide the transmitter which part of the data should be transmitted and enable the receiver to decode the transmitted information. 

Recently, deep learning (DL) has been widely integrated into task-oriented communication systems to establish the shared KB, which involves in joint training of transmitter and receiver on a huge of data samples in an end-to-end manner. Specifially, the transceivers are modeled as two deep neural networks (DNNs), where the transmitter is trained to extract a compact and informative representation of the input data, while the receiver is trained to decode the transmitted information based on the extracted representation. The gradient-based optimization algorithms, such as stochastic gradient descent (SGD) and its variants, are employed to train the transceivers with an associated loss function. After training, the shared KB is implicitly preserved in the parameters of the transceiver DNNs. Such DL-based task-oriented communication systems have shown significantly advantages in terms of the tradeoff between the spectrum efficiency and task performance. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TBD need to add some references here to describe the state-of-the-art work in this area.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Typically a deep neural network (DNN) is employed to model the transmitter and receiver, which can be trained using gradient-based optimization algorithms, such as stochastic gradient descent (SGD) and its variants. The DL-based task-oriented communication systems have shown significantly advantages in terms of the tradeoff between the spectrum efficiency and task performance, compared with traditional communication systems. However, the practical deployment of DL-based task-oriented communication systems faces several challenges, including the data-driven nature of DL, the high communication overhead induced by gradient-based optimization algorithms, and the susceptibility to distribution shifts.

% Due to the shared KB between transceivers, the DL-based task-oriented communication systems have shown significantly advantages in terms of the tradeoff between the spectrum efficiency and task performance, compared with traditional communication systems. 



Unless the existing magazine or survey literature, such as~\cite{jiang2023wireless} and~~\cite{gunduz2022beyond}, this paper focuses on the practical deployment challenges in DL-based task-oriented communication systems, \textcolor{red}{TBD}.

These challenges stem from the data-driven nature of DL, the high communication overhead induced by gradient-based optimization algorithms. Specifially, local training refers to the scenario where the shared KB in transceivers is established in a centralized manner. In contrast, remote training refers to when the transmitter and receiver locate in different places, where the training process involves the communication of the intermediate features and gradients between the transmitter and receiver. We first introduce the three training strategies for DL-based task-oriented communication systems. Next, we discuss the challenges in practical deployment of DL-based task-oriented communcation systems. Furthermore, we conduct two case studies to demonstrate the effectiveness of the proposed solutions for handling the above challenges. Eventually, open research issues and potential future directions are discussed to inspire further research.

The remainder of this paper is organized as follows. The next section discusses an overview of the training and inference process in DL-based task-oriented communication systems and highlight the challenges in practical deployment. In section~\ref{sec:method}, we discuss the potential solutions for addressing the above challenges.

\textcolor{red}{TBD}.

\begin{table*}[t]
    % \caption{COMPARISON OF THREE Training AND TRAINING METHODS FOR DL-BASED TASK-ORIENTED COMMUNICATION SYSTEMS}
    \caption{Comparison of three training strategies for DL-based task-oriented communication systems}
    \label{tab:1}
    \centering{}\includegraphics[width=17.5cm]{image/draw.pdf}
\end{table*}


% 三种方案对比：模型更新的成本很低时，比如发射器和接收器的参数trained in a centrailized manner before deployment，可以有第一个方案
% 1)全部本地训练并在部署前将模型传递给发射器和接收器； 这种方式是代价最小的，但是这种方案并不实际，因为在实际部署中，发射器和接收器往往是分布在不同的地方，因此我们需要在部署前将模型传递给发射器和接收器。
% 2)部署后在发射端或接收端进行本地训练，然后将模型传递给另一端；这种方式实际上代价会比较大，尤其是模型中线性层较多时，因为模型中很多高维矩阵需要传递。例如我们的收发器中各有一个1024*524和524*1024的矩阵，这样总参数量已经非常大了。另一方面，这需要我们在设计深度学习网络的时候让每一层，至少是每一个线性层的维度都尽可能的小，这种设计方案会掣肘模型的性能。
% 3)部署后发射端和接收端进行远程训练，传递中间特征和梯度；这种方式实际上代价不会很大，由于链式法则的存在，因为只需要传递中间层的特征和梯度，而不需要传递整个模型的参数。这种方式的代价主要来源于高频率的前向传播和反向传播。然而我们可以轻易的通过增加batch size来减少这部分代价，因此可以灵活的在通信代价和计算代价中进行权衡。另一方面，这种方式的不会对模型的设计产生非常大的限制，因为我们只需要限制中间层的维度，而不需要限制整个模型的维度。



% 注意，第二个办法可能还是最有效的，需要在cons和pros里面写清楚，第二个和第三个办法各自的优缺点以及适用场景。



% 需要声明，local training然后发送模型看起来是一个较优秀的策略，但实际上并不是，我们可以做一个简单的计算。
% 以resnet为例，参数量25.6M = 2560 0000，如果在小数据集上训练或者微调, 同时增大batch size，是可以做到比25.6M要小的浮点数数量的




%%%%%% 要总结所有的问题都是来源于deep learning, 一个是依赖数据，一个是需要大量的梯度计算。这两个性质给dl-based task-oriented communication带来了两个问题，分别是如何进行efficient training以及如何保证robust inference performance

%%%%%% 要从training和inference两个角度来讨论，efficient training和robust inference performance




% 3个图+一个表+2个结果图
% 1.第一个图是deep learning-semantic communication/task-oriented communication的工作的流程，包括training和inference。其中training又包括两种，local training, remote training两种范式。（formulate the system model)
% 2画一个表格，写清楚之前的task-oriented communication系统和我们提出的task-oriented communication系统有哪些不一样，点出之前task-oriented communication系统存在的问题，以及我们在新系统中提出的对应的解决方案
% 表格的话，我觉得可以把上面的三种方案写在表格里面，然后对比一下各自的优缺点。
% 3.画一下generalization，detection，channel robustness的示意图
% 4.画一下feature alignment的示意图

==> section/method.tex <==
\section{Design Framework for DL-based Task-oriented Communication Systems}
\label{sec:method}
% In this seciton, we present design frameworks to tackle the challenges in deploying deep learning-based task-oriented communication systems. Specifically
In this section, we present design frameworks for efficient training and robust inference performance in DL-based task-oriented communication systems, including:
% to address the challenges in deploying DL-based task-oriented communication systems. Specifially, we discuss advanced techniques for efficient training and robust performance enhancement, aiming to improve the system's adaptability and generalization capability, including:
\begin{itemize}
    \item Hybrid training strategy that combines the advantages of local training and remote training to achieve efficient training with low communication overhead.
    \item Feature alignment mechanism to enable training-free adaptation.
    \item Advanced out-of-distribution generalization and detection techniques to tackle data-distribution shift problem.
    \item Robust channel adaptation strategies to mitigate channel-distribution shift.
\end{itemize}

\subsection{Efficient Training Strategies}
\textit{1) Hybrid Framework for Single Transceiver Training:} As mentioned in Section~\ref{sec:problem}, post-deployment local training and remote training methods are generally more practical in real-world task-oriented communication systems, as the pre-deployment local training approach often requires a centralized setup where both the transmitter and receiver are co-located before deployment, which is rarely feasible. However, both post-deployment local training and remote training face significant communication overhead challenges. Local training demands the transfer of large model parameters between devices, while remote training involves frequent exchanges of intermediate features and gradients, both of which can strain communication resources in bandwidth-limited environments. To address these challenges, we propose a \textit{hybrid training framework} that combines the benefits of both local and remote training while reducing communication overhead and preserving system performance.

The proposed hybrid framework operates in two sequential stages: \textit{self-supervised local training} followed by \textit{supervised remote training}. In the \textit{self-supervised local training} phase, the transmitter independently trains on its local data using a self-supervised learning approach. This stage focuses on extracting a task-agnostic and compact representation (or abstract) of the input data without requiring ground-truth labels, allowing the model to learn generic feature representations that are broadly useful across different tasks. The use of self-supervised learning at this stage is particularly advantageous as it minimizes data annotation requirements and reduces the need for extensive communication between devices during the initial training phase.

Following this, the \textit{supervised remote training} phase involves fine-tuning the transmitter and receiver jointly by exchanging the intermediate features and gradients, enabling the system to specialize for the specific task with labeled data. By building on the task-agnostic representations learned during the local training phase, the remote fine-tuning process requires fewer gradient updates and feature exchanges, thereby significantly reducing communication overhead. Additionally, this two-stage approach allows the system to balance between computation and communication costs effectively. The self-supervised local training handles data-driven feature extraction with minimal communication, while the remote supervised training ensures task-specific refinement with minimal data transfer requirements.

This hybrid approach not only improves communication efficiency but also enhances system adaptability by enabling incremental updates as new data arrives. The framework is particularly suitable for dynamic environments where continuous model refinement is required without frequent full model parameter transfers. By integrating self-supervised learning and remote fine-tuning, the hybrid framework offers a scalable and practical solution for deep learning-based task-oriented communication systems.

\textit{2) Feature Alignment for Training-Free Cross-Transceiver Communication}:
DL-based task-oriented communication systems are often designed and trained in a point-to-point fashion, where each transceiver pair is independently optimized to maximize task performance. However, this isolated training paradigm often leads to incompatible feature representations among individually training transceiver paris, even on the same dataset, preventing effective communication over wireless networks. This arises from the isolated gradient optimization process based on their initialization and optimization paths, lead to feature misalignment across different transceiver pairs. As a result, one transmitter cannot effectively communicate with a receiver trained in isolation, or need to be retrained or fine-tuned to adapt to the receiver's feature space under the \textit{remote training} framework, limiting the system's generalizability and scalability in multi-user scenarios.


To overcome this challenge, we propose a \textit{training-free} \textit{feature alignment} method designed to enable seamless cross-transceiver communication by leveraging a set of shared anchor data samples across all transceiver pairs. These anchor data points, included in the training datasets of all transceivers, serve as a common reference for feature space calibration. The core idea is based on \textit{angle preserving} and \textit{linear invariance} assumption. Specifially, \textit{angle preserving} assumption states that the angle of two encoded features is same across different encoders, while \textit{linear invariance} assumption states that each pair of encoded feature by two different encoders comes from one linear transformation.

% that the relateive feature representations among anchor data samples and any other data points should be consistent across different transceivers.
% The core idea is to ensure that the encoded feature representations generated by different transceivers for the same anchor data points remain closely aligned. 
% To further enhance this alignment, we introduce a \textit{transformation matrix} during training, which is optimized to project the feature spaces of different transceivers into a shared latent space, minimizing the distance between their respective feature representations.
Based on these two assumptions, we propose two complementary \textit{feature alignment frameworks} tailored for both the \textit{transmitter-side} and the \textit{receiver-side} alignment:

\begin{itemize}
    \item \textbf{Transmitter-Side Alignment}: By leveraging the \textit{angle preserving} assumption~\cite{}, the transmitter's encoder is trained to transmit relateive feature angle of input data samples upon anchor data samples, and the receiver will leverage the relative anlge information instead of the absolute feature values to decode for further inference. 
    \item \textbf{Receiver-Side Alignment}: By leveraging the \textit{linear invariance} assumption, the receiver side can estimate the transformation matrix based on the received features of the anchor data samples. The estimation of transformation matrix can either be done by learning-based method or closed-form solution from Least Square (LS) and Minimum Mean Square Error (MMSE) methods.
\end{itemize}

By employing the proposed feature alignment approach, we can achieve training-free cross-transceiver communication, significantly enhancing the interoperability of task-oriented communication systems. This approach eliminates the need for full model retraining when introducing new transceivers, making it ideal for dynamic, large-scale networks where multiple transmitters and receivers must interact seamlessly. Additionally, the shared anchor-based alignment strategy improves the system's robustness to data variations and initialization differences, further contributing to its scalability and generalization capacity. 


\subsection{Robust Inference Strategies}
\textit{1) Robust Strategies to Data Distribution Shift:}
As DL-based task-oriented communication system often faces the challenge of data-distribution shift, where the input data during testing may differ significantly from the data used during training, leading to performance degradation or even system failure. To address this issue, we propose a data-invariant feature extraction strategy based on \textit{information bottleneck} (IB) principle and \textit{invariant risk minimization} (IRM). The IB framework helps the transceiver system focus on the most informative and compact representations by minimizing the mutual informtation between the input data and the learned feature representation while maximizing the mutual information between the feature representation and the ground truth. Complementing this, the IRM principle encourages the transceiver to learn causal features across diverse training distributions, ensuring the learned features remain stable even when the input distribution changes.

Our approach involves training the transmitter and receiver using multiple domains or data sources where a shared invariant feature set is identified and optimized. By enforcing constraints that penalize reliance on domain-specific features features, the model learns to extract minimal and causal representations and generalize better to unseen conditions. Furthermore, \textit{out-of-distribution} (OoD) detection mechanisms can be integrated to reject to make inference when unknown data category is involved, where confidence scores based on feature divergence can trigger mechanisms like uncertainty-aware decision making or request retransmissions when confidence drops below a threshold. 

By employing a combination of IB, IRM and OoD detection, the proposed robust inference strategy enhances the systems' generalization capability and reliability even when faced with unexpected data variations. This approach is particularly beneficial in dynamic wireless environments where the transmitted data often varies due to changing contexts or user behaviors.

\textit{2) Robust Strategies to Channel Distribution Shift:}
Except for data distribution shift, channel distribution shift is another critical challenge in DL-based task-oriented communication systems, where the test SNR conditions differ from the training SNR conditions. SInce varying channel conditions can significantly impact the reliability of both feature transmission and task performance, conventional training under fixed SNR or a specific range of SNR values may not be sufficient to ensure robust performance in real-world scenarios. Furthermore, such variations can not be solved by previous data-invariant feature extraction strategies, as there is no causal relationship between the input data and the channel conditions. 

To address above issue, we propose a \textit{Hypernetwork}-based adaptive joint source channel coding approach for channel-aware feature adaptation. Specifially, by only introducing a minimal extra \textit{hypernetwork} architecture, the model can dynamically generate part of the parameters in the transceiver model based on the real-time SNR conditions, instead of relying on a fixed model optimized for a specific SNR set. During training, the hypernetwork is conditioned on multiple SNR levels, enabling it to learn a continuous mapping between channel quality and optimal feature encoding.
Such strategy enable the task-oriented communication system to adapt to varying channel conditions without retraining the entire model, within a small computational overhead. 

The primary advantage of this approach lies in its compact design and scalability, as a single model can be deployed across varying channel conditions without the need to store separate models for different SNR regimes. Furthermore, by dynamically adapting to channel conditions, Hyper-AJSCC minimizes both task performance degradation and communication overhead, achieving a more reliable and efficient task-oriented communication system. This method not only enhances the system's robustness to channel variations but also contributes to the broader goal of \textit{efficient training}, where transceivers can maintain high-performance inference without frequent model retraining or manual reconfiguration.




% To address above issue, we propose a \textit{training-free} \textit{feature alignment} method designed to ensure cross-transceiver by leveraging shared anchored data among isolated training transceiver pairs. A set of anchor data samples is included in all transceiver training dataset, which serves as a common reference point for feature alignment. To ensure the cross-transceiver feature alignment, we further introduce a transformation matrix to align the feature space of different transceivers. We design two frameworks for feature alignment for transmitter side and receiver side. Specifially, for the receiver side, 





% As mentioned in Section~\ref{sec:problem}, the post-deployment local training and remote training methods are more practical in real-world scenarios, while the pre-deployment local training method is not always feasible due to the requirement for centralized transmitter and receiver. However, both methods suffer from high communication overhead during training. To address this issue, we propose a hybrid training framework that combines the advantages of local training and remote training, aiming to reduce the communication overhead while maintaining the systems's performance. 

% The hybrid training framework consists of two stages: 1) self-supervised local training and 2) supervised remote training. Specifially, in the local training stage, the transmitter perform self-supervised training using its local data samples. Such self-supervised training strategy aims to extract a task-agnostic \textit{abstract} of the input data and do not require the knowledge of ground-truth labels. 


% In the local training stage, the transmitter and receiver perform independent training using their local data samples. The transmitter extracts intermediate features from the input data and sends them to the receiver, which decodes the transmitted information based on the received features. The transmitter and receiver update their model parameters based on the local data samples and the received features, respectively. In the remote training stage, the transmitter and receiver exchange intermediate features and gradients to jointly optimize the model parameters. The transmitter and receiver update their model parameters based on the received features and gradients, respectively. The hybrid training framework is illustrated in Fig.~\ref{fig:framework}(a), where the transmitter and receiver perform local training and remote training iteratively to optimize the model parameters. This hybrid training strategy aims to reduce the communication overhead while maintaining the system's adaptability and robustness.



% As mentioned in Section~\ref{sec:problem}, the local training (post-deployment) and remote training methods are more practical in real-world scenarios. However, both methods suffer from high communication overhead during training. To address this issue, we propose a hybrid training framework that combines the advantages of local training and remote training, aiming to reduce the communication overhead while maintaining the system's adaptability and robustness. Specifically, the hybrid training framework consists of two stages: local training and remote training. In the local training stage, the transmitter and receiver perform independent training using their local data samples. The transmitter extracts intermediate features from the input data and sends them to the receiver, which decodes the transmitted information based on the received features. The transmitter and receiver update their model parameters based on the local data samples and the received features, respectively. In the remote training stage, the transmitter and receiver exchange intermediate features and gradients to jointly optimize the model parameters. The transmitter and receiver update their model parameters based on the received features and gradients, respectively. The hybrid training framework is illustrated in Fig.~\ref{fig:framework}(a), where the transmitter and receiver perform local training and remote training iteratively to optimize the model parameters. This hybrid training strategy aims to reduce the communication overhead while maintaining the system's adaptability and robustness.


% a design framework to address the challenges in deploying deep learning-based task-oriented communication systems. Specifically, we propose a novel training strategy that combines the advantages of local training and remote training, aiming to reduce the communication overhead while maintaining the system's adaptability and robustness. We also introduce a feature alignment mechanism to enhance the generalization capability of the system and improve its performance under distribution shifts. The proposed design framework is illustrated in Fig.~\ref{fig:framework}, which consists of three key components: 1) a hybrid training strategy, 2) a feature alignment mechanism, and 3) a robustness enhancement module. We describe each component in detail below.

==> section/problem.tex <==
\section{Training strategies and Challenges in DL-based Task-oriented Communication Systems}
\label{sec:problem}

In this section, we first discuss the training strategies of DL-based task-oriented communication system. Then, we highlight the challenges in these strategies and the inference process. 
\subsection{Three Training Strategies for DL-based Task-oriented Communication Systems}
Table~\ref{tab:1} compares three training and deployment methods for deep learning-based task-oriented communication systems: Local Training (Pre-deployment), Local Training (Post-deployment), and Remote Training. Each method has distinct advantages and limitations, particularly in terms of practicality, communication overhead, and adaptability.

\textbf{Local Training (Pre-deployment)} involves training the model centrally before deployment and distributing the model parameters to both transmitter and receiver. This approach is straightforward, optimally leverages centralized training resources, and simplifies model architecture design. However, it becomes impractical if the transmitter and receiver are physically separated and does not allow further adaptation to real-world conditions after deployment without re-transferring the model.

\textbf{Local Training (Post-deployment)} allows one side (e.g., the transmitter or receiver) to perform local training after deployment and then transfer the trained model parameters to the other side. A notable advantage is that the model parameters only need to be transferred once, reducing the number of updates. However, this method can incur high communication costs, especially when the model includes large linear layers with high-dimensional matrices. Furthermore, designing the model requires lightweight architecture considerations, which may constrain performance. Like the pre-deployment method, further adaptation after deployment would require another model transfer.

\textbf{Remote Training} addresses these limitations by enabling joint training of the transmitter and receiver through the exchange of intermediate features and gradients, instead of the entire model. This approach avoids transferring large parameters, allows adaptability after deployment,  especially fine-tuning the model when new data is available. However, this method requires frequent forward and backward passes over wireless channels, which incurs a tradeoff between communication overhead and system performance.


\subsection{Challenges in the Deployment of DL-based Task-oriented Communication Systems}

% \textbf{Data-Distribution Shift:} One of the fundamental challenges in deploying deep learning-based task-oriented communication systems is the issue of data-distribution shift, where the input data during testing may differ significantly from the data used during training. This often occurs in real-world scenarios due to dynamic environments, unpredictable input variations, or changes in task-related contexts. For instance, a system trained on data from a specific domain (e.g., clear images or standardized text) may experience significant performance degradation when deployed in a different domain (e.g., low-quality images or unseen textual patterns). Such shifts undermine the generalization capability of deep learning models, as they tend to overfit to the training data. Addressing this problem requires the integration of robust out-of-distribution detection mechanisms, domain adaptation techniques, or invariant feature extraction strategies to ensure the system maintains reliable performance when confronted with data variations.

% \textbf{Channel-Distribution Shift:} Another critical challenge arises from the channel-distribution shift, which refers to changes in the Signal-to-Noise Ratio (SNR) during deployment compared to the SNR conditions used during training. In practical wireless communication systems, the channel conditions are inherently dynamic, with the SNR often fluctuating due to environmental factors, interference, or user mobility. Deep learning models trained under specific SNR values may fail to adapt effectively when exposed to different SNR conditions during testing, leading to degraded communication efficiency and task performance. To mitigate this issue, solutions such as SNR-aware training, adaptive coding strategies, and robust feature extraction methods can be employed. Additionally, techniques like dynamic SNR adaptation or hypernetwork-based modulation can enhance the model’s ability to generalize across varying channel conditions.

\textbf{Distribution Shift:} A fundamental challenge in deploying deep learning-based task-oriented communication systems is the issue of \textit{distribution shift}, which occurs when the input data or channel conditions during deployment differ from those observed during training. \textit{Data-distribution shift} arises when the testing data diverges from the training data, often due to dynamic environments, unpredictable variations, or domain changes. For instance, a model trained on clear images or standardized text may experience degraded performance when tested on low-quality inputs or previously unseen patterns. Similarly, \textit{channel-distribution shift} refers to the variation in Signal-to-Noise Ratio (SNR) during deployment compared to the training phase, commonly caused by dynamic wireless conditions, interference, or user mobility. These shifts can undermine the generalization capability of deep learning models, leading to overfitting or degraded task performance. Addressing distribution shifts requires the integration of robust out-of-distribution detection mechanisms, domain adaptation techniques, and invariant feature extraction methods to improve resilience against data variations. Additionally, SNR-aware training, adaptive coding strategies, and dynamic SNR adaptation techniques can be employed to ensure stable performance across varying channel conditions.

\textbf{High communication Overhead During Training:} 
As the pre-deployment local training method is not always feasible, the post-deployment local training and remote training methods are more practical in real-world scenario. But both methods have the challenges of high communication overhead during training. For local training (post-deployment), transferring the entire model parameters from one side (e.g., transmitter) to the other (e.g., receiver) side can be costly, especially when the model includes large linear layers with high-dimensional matrices. This overhead increases the latency and consumes significant communication resources. On the other hand, remote training, which involves frequent exchange of intermediate features and gradients, introduces additional communication costs due to the iterative forward and backward passes required for gradient-based optimization. To address these challenges, lightweight model designs, gradient compression, and dimensionality reduction of intermediate features can be explored to reduce overhead. Furthermore, methods such as batch-size adjustment and adaptive training strategies can help balance communication and computation costs, making the system more efficient for real-world deployment.

==> section/simulation.tex <==
\section{Case studies}
\label{sec:case studies}
